Scaling Survival Analysis in Healthcare with Federated Survival Forests: A Comparative Study on Heart Failure and Breast Cancer Genomics

Survival analysis is a fundamental tool in medicine, modeling the time until an event of interest occurs in a population. However, in real-world applications, survival data are often incomplete, censored, distributed, and confidential, especially in healthcare settings where privacy is critical. The scarcity of data can severely limit the scalability of survival models to distributed applications that rely on large data pools. Federated learning is a promising technique that enables machine learning models to be trained on multiple datasets without compromising user privacy, making it particularly well-suited for addressing the challenges of survival data and large-scale survival applications. Despite significant developments in federated learning for classification and regression, many directions remain unexplored in the context of survival analysis. In this work, we propose an extension of the Federated Survival Forest algorithm, called FedSurF++. This federated ensemble method constructs random survival forests in heterogeneous federations. Specifically, we investigate several new tree sampling methods from client forests and compare the results with state-of-the-art survival models based on neural networks. The key advantage of FedSurF++ is its ability to achieve comparable performance to existing methods while requiring only a single communication round to complete. The extensive empirical investigation results in a significant improvement from the algorithmic and privacy preservation perspectives, making the original FedSurF algorithm more efficient, robust, and private. We also present results on two real-world datasets demonstrating the success of FedSurF++ in real-world healthcare studies. Our results underscore the potential of FedSurF++ to improve the scalability and effectiveness of survival analysis in distributed settings while preserving user privacy.

==> het.tex <==
\begin{table}[t]
    \centering
    \caption{Heterogeneity score $h$~\cite{archetti2023heterogeneous} for each dataset in the experiments. $K$ is the number of clients in the federation for each dataset. $\alpha$ is the splitting parameter for the label-skewed algorithm~\cite{archetti2023heterogeneous} to simulate federations for centralized datasets.}
    \label{tab:heterogeneity}
    
    \begin{tabularx}{\linewidth}{@{} l Y Y Y Y @{}}
        \toprule
        \textbf{Dataset} & \textbf{$K$} & \textbf{$\alpha$} & \textbf{$h$} \\
        \midrule
        WHAS500~\cite{hosmer_applied_2008} & 10 & 5.0 & 13.3\%\\
        GBSG2~\cite{schumacher1994randomized} & 10 & 5.0 & 11.1\%\\
        METABRIC~\cite{pereira_somatic_2016,katzman2018deepsurv} & 10 & 5.0 & 60.0\%\\
        NWTCO~\cite{breslow_design_1999} & 10 & 5.0 & 71.1\%\\
        FLCHAIN~\cite{therneau2023survival} & 10 & 5.0 & 75.6\%\\
        \bottomrule
    \end{tabularx}
\end{table}

